Large-Scale Dataset Pruning in Adversarial Training through Data Importance Extrapolation

Their vulnerability to small, imperceptible attacks limits the adoption of deep learning models to real-world systems. Adversarial training has proven to be one of the most promising strategies against these attacks, at the expense of a substantial increase in training time. With the ongoing trend of integrating large-scale synthetic data this is only expected to increase even further. Thus, the need for data-centric approaches that reduce the number of training samples while maintaining accuracy and robustness arises. While data pruning and active learning are prominent research topics in deep learning, they are as of now largely unexplored in the adversarial training literature. We address this gap and propose a new data pruning strategy based on extrapolating data importance scores from a small set of data to a larger set. In an empirical evaluation, we demonstrate that extrapolation-based pruning can efficiently reduce dataset size while maintaining robustness.

==> acronyms.tex <==

\begin{acronym}
    \acro{APGD}{Auto-\ac{PGD}}
    \acro{CNN}{Convolutional Neural Network}
    \acro{DDPM}{Denoising Diffusion Probabilistic Model}
    \acro{DFT}{Discrete Fourier Transform}
    \acro{DL}{Deep Learning}
    \acro{DLR}{Difference of Logits Ratio}
    \acro{DNN}{Deep Neural Network}
    \acro{DU}{Dynamic Uncertainty}
    \acro{EDM}{Elucidating Diffusion Model}
    \acro{EDU}{Extrapolated \ac{DU}}
    \acro{EFP}{Extrapolated \ac{FP}}
    \acro{FAB}{Fast Adaptive Boundary}
    \acro{FFP}{Fundamental Frequency Pruning}
    \acro{FFT}{Fast Fourier Transform}
    \acro{FID}{Frechet Inception Distance}
    \acro{FP}{Frequency Pruning}
    \acro{GAN}{Generative Adversarial Network}
    \acro{GLISTER}{GeneraLIzation based data Subset selecTion for Efficient and Robust learning}
    \acro{GT}{Ground Truth}
    \acro{IDBH}{Improved Diversity and Balanced Hardness}
    \acro{KNN}{K-Nearest Neighbors}
    \acro{MAE}{Mean Absolute Error}
    \acro{MART}{Misclassification Aware adveRsarial Training}
    \acro{ML}{Machine Learning}
    \acro{MLP}{Multilayer Perceptron}
    \acro{NN}{Neural Network}
    \acro{PGD}{Projected Gradient Descent}
    \acro{ResNet}{Residual Neural Network}
    \acro{SGD}{Stochastic Gradient Descent}
    \acro{SOTA}{State Of The Art}
    \acro{SSCD}{Self Supervised Copy Detection}
    \acro{SVM}{Support Vector Machine}
    \acro{SWA}{Stochastic Weight Averaging}
    \acro{TRADES}{TRadeoff-inspired Adversarial DEfense via Surrogate-loss minimization}
    \acro{VAE}{Variational Autoencoder}
    \acro{ViT}{Vision Transformer}
    \acro{AA}{AutoAttack}
    % add your acronyms here
\end{acronym}

